Information Theoretic Model Predictive Control: Theory and Applications to Autonomous Driving

We present an information theoretic approach to stochastic optimal control problems that can be used to derive general sampling based optimization schemes. This new mathematical method is used to develop a sampling based model predictive control algorithm. We apply this information theoretic model predictive control (IT-MPC) scheme to the task of aggressive autonomous driving around a dirt test track, and compare its performance to a model predictive control version of the cross-entropy method.

==> Sections/information-theoretic-mppi.tex <==
In section \ref{it-control} we developed a formula for computing an optimal open loop control sequence which corresponds to taking a cost-weighed average over sampled trajectories. In this section we take this development further and show how this can be utilized in a model predictive control framework. There are four main issues with adapting \eqref{Equation:IT-Controls} to model predictive control that we address in this section:
% * <jimrehg@gmail.com> 2017-06-26T05:52:13.489Z:
% 
% > open loop control sequence
% In Section III I think we could be benefit from stating more explicitly that we are developing an open loop control law. This was mentioned as an aside in a few places, but I think it would be useful to state it up-front and also briefly describe the difference with the closed loop approach that can foreshadow this section (so the reader has a better sense of where we will be going).
% 
% ^.
\begin{enumerate}
\item De-coupling the temperature and control cost terms
\item Handling control constraints
\item Control Smoothing
\item Sampling trajectories in real-time
\end{enumerate}
The mathematical framework that we will utilize in developing our solution to these issues is the information-theoretic framework presented in section~\ref{it-control}. However, due to the close mathematical relationship that this framework has with previous methods developed purely in the path integral control framework, we will refer to the resulting control algorithm  as information-theoretic model predictive path integral control (IT-MPPI).

\subsection{Decoupling control cost and temperature}

Consider the form of the importance sampling weight from \eqref{Equation:IT-Controls} when we take the uncontrolled dynamics of the system as the base distribution:\footnote{This is a natural choice from an optimization perspective, since the minimum control cost is achieved with $U \equiv {\bf{0}}$.}
\begin{equation}
w(\mathcal{E}) = \exp\left( -\frac{1}{\lambda} \left( S(\mathcal{E}) + \lambda \sum_{t=0}^{T-1} \vu^\rT \Sigma^{-1} \epsilon_t \right) \right). \nonumber
\end{equation}
The challenge with this formulation is that changing the inverse temperature $\lambda$, also changes the relative control cost and vice versa. This is sensible from a theoretical point of view: If we are allowed more control authority over the system, then we should be able to more tightly maintain a given trajectory, which means that the optimal distribution is narrower. Raising the temperature in the softmax achieves this by creating a more highly peaked distribution. However, in a practical real-time setting this is problematic. Raising the temperature too high results in numerical instability since most trajectories are numerically annihilated, at which point the importance sampling oscillates between solutions instead of converging. Our solution is to change the base distribution which defines the control cost. Let $\bar{U}$ be the current planned control sequence, and define the new base distribution as:
% * <jimrehg@gmail.com> 2017-06-26T06:10:21.223Z:
% 
% > numerically annihilated
% I don't understand what this phrase means. Some more discussion is needed for this to be clear. Perhaps you can make a plot showing the effect of temperature? Or if this is a standard phenomena perhaps you can site a plot in another article that is illustrative?
% 
% ^.
% * <jimrehg@gmail.com> 2017-06-26T06:07:55.463Z:
% 
% > optimal distribution is narrower
% The effect of the inverse temperature on the solution has not been discussed until now. I think a sentence or two should be added to section III making it clear what \lambda does. Then this sentence will also be clear.
% 
% ^.
\begin{equation}
\tilde{p}(V) = p(V|\alpha\bar{U}, \Sigma), \nonumber
\end{equation}
where $0 < \alpha < 1$. With $\alpha=0$, the base distribution reverts back to the uncontrolled dynamics and pushes $U$ to zero. And with $\alpha = 1$, the base distribution is the distribution corresponding to the current planned control law, which keeps $U$ near the distribution corresponding to $\bar{U}$. The case of $\alpha=1$ can be interpreted as placing a cost on how much the new open loop control law is allowed to deviate from the previous one, which is useful for creating smooth motions. A value in-between zero and one balances the two requirements of low energy and smoothness.

The construction of the optimal distribution and the corresponding control law are the same under this new base distribution. However, the control cost portion of the importance sampling weight now becomes:
\begin{equation}
\sum_{t=0}^{T-1} (1 - \alpha) \bar{\vu}_t^\rT \Sigma^{-1} \vv_t + (1 - \alpha^2)\bar{\vu}^\rT \Sigma^{-1} \bar{\vu}.\nonumber
\end{equation}
This can be further simplified by noting that $(1 - \alpha^2)\bar{\vu}^\rT \Sigma^{-1} \bar{\vu}$ does not depend on the optimized trajectory, yielding
\begin{equation}
w(\mathcal{E}) = \exp(-\frac{1}{\lambda}\left(S(\mathcal{E}) + \lambda (1-\alpha) \sum_{t=0}^{T-1} \vu^\rT \Sigma^{-1} \mathcal{\epsilon} \right). \nonumber
\end{equation}
Since $0 < \alpha < 1$ is a free parameter, we can choose $\gamma < \lambda$ as the new control cost parameter, resulting in
% * <jimrehg@gmail.com> 2017-06-26T06:22:14.335Z:
% 
% > a free parameter, we can choose $\gamma < \lambda$
% This is confusing. First \alpha maybe a free parameter but how close it is to 0 or 1 would seem to matter based on the discussion above. It seems like you are just setting \gamma = \lambda(1-\alpha) but then why is this inequality the motivation for this choice? Is this true for some other reason or it just follows from the choice of \gamma?
% 
% ^.
\begin{equation}
w(\mathcal{E}) = \frac{1}{\eta}\exp\left(-\frac{1}{\lambda}\left(S(\mathcal{E}) + \gamma \sum_{t=0}^{T-1} \vu^\rT \Sigma^{-1} \mathcal{\epsilon} \right)\right),\nonumber
\end{equation}
as the final probability weighting for the algorithm. Note that the control cost term $\gamma \sum_{t=0}^{T-1} \vu^\rT \Sigma^{-1} \epsilon_t$ always penalizes controls away from ${\bf{0}}$, not from the apparent target $\alpha \bar{U}$. The sampling procedure implicitly penalizes deviations away from $\bar{U}$ and the two competing penalties (one explicit and one implicit) reach an equilibrium at $\alpha \bar{U}$.

\subsection{Handling Control Constraints} \label{sec:control-constraints}

Most interesting control systems, including the autonomous vehicle we consider here, have actuator limits that the controller must take into account. There are several ways to do this in our information theoretic framework: annihilating trajectories that violate the control constraints, or by formulating the optimization problem in \eqref{Equation:QuadraticMin} as a quadratic program and solving the constrained optimization problem.
% * <jimrehg@gmail.com> 2017-06-26T06:26:08.033Z:
% 
% > annihilating trajectories
% You seem to like using this word but as far as I know it is not a technical term. Are you just referring to rejection sampling here?
% 
% ^.

Although both of these methods could work in theory, they both have significant drawbacks in practice. The first approach completely removes trajectory samples from the optimization, and the second one requires solving a quadratic program online. A simpler solution is to make the problem unconstrained by pushing the control constraints into the system dynamics: 
% * <jimrehg@gmail.com> 2017-06-26T06:29:19.348Z:
% 
% > completely removes trajectory samples from the optimization
% It's not a priori clear why this is a  bad thing. If you are talking about rejection sampling then the precise argument is that it makes the sampler potentially very inefficient.
% 
% ^.
\begin{equation}
\vx_{t+1} = \vF(\vx_t, g(\vv_t)), \nonumber
\end{equation}
where $g(\vv_t)$ is a clamping function that restricts $\vv_t$ to remain within an allowable input region. Since the IT-MPPI controller does not require any linearization of the dynamics, adding this additional non-linearity is trivial to implement and works well in practice. 

\subsection{Control Smoothing}

The stochastic nature of the sampling procedure can lead to significant chattering in the resulting control, which can be removed by smoothing the output control sequence. One very effective method for smoothing is by fitting local polynomial approximations to the control sequence. Consider the quadratic objective \eqref{Equation:QuadraticMin}:
\begin{equation}
\label{Equation:StandardOpt}
\vu_t^* = \argmin\left( \ExP{\Qb^*}{\left(\vv_t - \vu_t\right)^\rT \Sigma^{-1}\left(\vv_t - \vu_t \right)} \right).
\end{equation}
And now consider fitting a local polynomial approximation (at every timestep) so that $\vu_t = \va_0 + \va_1t + \va_2t^2 + \dots \va_k t^k = A \vt$, where $A = (\va_0, \va_1, \dots \va_k)$ and $\vt = (1, t, t^2, \dots t^k)$. Our goal is now to find the optimal set of coefficients, at each timestep. The optimal coefficients, at timestep $j$, can be found through the following optimization:
\begin{equation}
A_j^* = \argmin\left( \ExP{\Qb^*}{\sum_{t = (j-k)}^{j+k} \left(\vv_t - A\vt \right)^\rT \Sigma^{-1}\left(\vv_t - A \vt \right)} \right).\nonumber \\
\end{equation}
Note how the optimization now spans multiple timesteps into the past and future in order to compute a smoother control input. This optimization problem is equivalent to optimizing the objective:
\begin{align}
&\ExP{\Qb^*}{\sum_{t = (j-k)}^{j+k} \vv_t^\rT \Sigma^{-1} A \vt + \vt^\rT A^\rT \Sigma^{-1} A \vt} \nonumber \\
&= \sum_{t = (j-k)}^{j+k} \ExP{\Qb^*}{\vv_t}^\rT \Sigma^{-1}  A \vt + \vt^\rT A^\rT \Sigma^{-1} A \vt. \nonumber
\end{align}
This in turn is equivalent to the minimization:
\begin{align}
\label{Equation:Smoothing}
\small{A_t = \argmin\left( \sum_{t = j-k}^{j+k} \left(\ExP{\Qb^*}{\vv_t} - A\vt \right)^\rT \Sigma^{-1}\left(\ExP{\vq^*}{\vv_t} - A \vt \right) \right)} \nonumber
\end{align}
This is a convenient expression because it means that we can first compute the weighted average over trajectories, and then perform a local polynomial approximation in order to smooth the resulting control sequence. In other words, we do not have to handle any polynomial expressions inside the expectation. The naive method for computing the controls is to then compute $\ExP{\Qb^*}{\vv_t}$ using a Monte-Carlo approximation, solve for each $A_t$, and lastly compute the smoothed control inputs $\vu_t$. However, a simpler method which achieves the same result is to use a Savitsky-Galoy filter \cite{savitzky1964smoothing} which implements local polynomial smoothing using a specific set of convolution coefficients. Using a Savitsky-Galoy filter, we simply compute $\tilde{U} = \ExP{\Qb^*}{V}$ and then compute the smoothed control sequence $U$ by passing $\tilde{U}$ through the convolutional filter.

\subsection{GPU-Based Trajectory Sampling}

The key requirement for the success of the IT-MPPI algorithm is the ability to generate and evaluate a large number of samples in real time. As in our prior sampling-based MPC method~\cite{williams2017model}, we perform sampling in parallel on a graphics processing unit (GPU) with Nvidia\textquotesingle s CUDA architecture. In our implementation, all of the trajectory samples are processed individually in parallel. In addition to the sample level parallelism, each individual sample uses between 4 and 16 CUDA threads depending on the dynamics model. This is done in order to take advantage of the parallel nature of the linear algebra routines that our vehicle dynamics models rely on. Depending upon the model and cost function, our implementation can achieve control loops from 40-60 HZ using a few thousand samples of 2-3 second long trajectories. Note that sampling 1200, 2.5 second long trajectories at 40 Hz corresponds to making approximately 4.8 million queries to the full non-linear dynamics of the vehicle every second. For the complex vehicle dynamics that we consider, this is only possible using a modern GPU. 

\subsection{Real-Time MPC Algorithm}

With our control update law for open loop sequences, as well as methods for handling control constraints, smoothing, and real-time sampling, we are now ready to describe the full IT-MPPI algorithm as well as the model predictive control version of the cross-entropy method. The basic sampling-based model predictive control algorithm (Alg. \ref{Algorithm:sb_mpc}) starts by taking in the current state from an external state estimator, and then produces $K$ trajectory samples in parallel on the GPU. Each sample is generated by randomly sampling a sequence of control perturbations, each drawn from $p(\bar{U}, \Sigma)$, then the dynamics are simulated forward, and the cost is computed for each trajectory.

Once the costs for each perturbation sequence are computed, they are converted to probability weights. In the IT-MPPI algorithm, this is done using the method in Alg. \ref{Algorithm:mppi}, and in the cross-entropy method this is done via the method in Alg. \ref{Algorithm:cem}. The difference between the two approaches is that the IT-MPPI method takes a weighted average over \emph{all} trajectory samples, and the cross-entropy method takes an un-weighted average over the top $\delta$ percentile of samples (usually $\delta > .75$).

Once the probability weights have been computed, the un-smoothed control update is performed by computing the probability weighted average over all the perturbation sequences. Lastly, this update is smoothed by passing it through a convolutional filter with the Savitsky-Galoy coefficients. The first control is sent to the actuators, and the remaining sequence of length $T-1$ is slid down and used to warm-start the optimization at the next time instance.

\begin{algorithm}
\SetKwInOut{Input}{Given}
\Input{$\vF, g$: Transition Model\;
       $K$: Number of samples\;
       $T$: Number of timesteps\;
       $(\vu_0, \vu_1, ... \vu_{T-1})$: Initial control sequence\;
       $\Sigma, \phi, q, \gamma, \alpha$: Cost functions/parameters\;
       $\text{SGF}$: Savitsky-Galoy convolutional filter\;}        
\While{task not completed}{
$\vx_0 \leftarrow \text{GetStateEstimate()}$\;
\For{$k \leftarrow 0$ \KwTo $K-1$}{
  $\vx \leftarrow \vx_0$\;
  Sample $\mathcal{E}^k = \left( \epsilon_0^k \dots \epsilon_{T-1}^k \right), ~\epsilon_t^k \in \mathcal{N}(0, \Sigma)$\;
  \For{$t \leftarrow 1$ \KwTo $T$}{
    \If{$k < (1 - \alpha) K$}{
    	$\vv_{t-1} = \vu_{t-1} + \epsilon_{t-1}^k$\;
    }\Else{
    	$\vv_{t-1} = \epsilon_{t-1}^k$\;
    }
    $\vx \leftarrow \vF(\vx, g(\vv_{t-1}))$\;
  	$S_k \pluseq  \vq(\vx) + \gamma \vu_{t-1}^\rT \Sigma^{-1} (\vu_t - \vv_t)$\;
  }
  $S_k \pluseq \phi(\vx)$\;
}

$\text{ComputeWeights}(S_0, S_1, \dots S_k)$\;
\For{$t \leftarrow 0$ \KwTo $T-1$}{
$U \leftarrow U + \text{SGF}*\left(\sum_{k=1}^K w_k \mathcal{E}^k\right)$\;
}

$\text{SendToActuators}(\vu_0)$\;

\For{$t \leftarrow 1$ \KwTo $T-1$}{ 
	$\vu_{t-1} \leftarrow \vu_t$\;  
}
$\vu_{T-1} \leftarrow \text{Intialize}(\vu_{T-1})$\;
}
\caption{Sampling Based MPC \label{Algorithm:sb_mpc}}
\end{algorithm}

\begin{algorithm}
\SetKwInOut{Input}{Given}
\Input{$S_1, S_2, \dots S_K$: Trajectory costs\;
$\lambda$: Inverse Temperature\;}
$\beta \leftarrow \min_k[ S_k) ]$\;
$\eta \leftarrow \sum_{k=1}^{K} \exp\left( -\frac{1}{\lambda} (S_k - \beta) \right)$\;
\For{$k \leftarrow 1$ \KwTo $K$}{
  $w_k \leftarrow \frac{1}{\eta}\exp\left( -\frac{1}{\lambda} (S_k - \beta) \right)$\;
}
\Return $\{w_1, w_2, \dots w_K \}$
\caption{Compute Weights (Information Theoretic) \label{Algorithm:mppi}}
\end{algorithm}

\begin{algorithm}
\SetKwInOut{Input}{Given}
\Input{$S_1, S_2, \dots S_K$: Trajectory costs\;
$\delta$: Eliteness Threshold\;}
$\zeta \leftarrow \text{round}(K(1 - \delta))$\;
$Z \leftarrow S_d$\;
\For{$k \leftarrow 1$ \KwTo $K$}{
  $w_k \leftarrow \frac{1}{\zeta}I\{S_k < Z\}$\;
}
\Return $\{w_1, w_2, \dots w_K \}$
\caption{Compute Weights (Cross Entropy) \label{Algorithm:cem}}
\end{algorithm}

The iterative importance sampling procedure, where trajectories are sampled using the un-executed portion from the previously computed sequence is key to achieving a high level of performance with the algorithm. However, in the presence of strong disturbances the importance sampling procedure can be problematic. This is because an exceptionally strong disturbance (see Fig.\ref{Fig:Disturbances}) can push the entire spray of trajectories into low cost regions where it may be impossible to recover. As a solution, we maintain a very small (less than one percent) number trajectories which do not use any importance sampler (i.e they are just Gaussian perturbations around zero). This enables the IT-MPPI algorithm to reset itself if a disturbance destroys the effectiveness of the previously computed control, and as long as the proper importance sampling weight is included it does not bias the estimate of the optimal control sequence.

